On Quantifying and Understanding the Role of Ethics in AI Research: A Historical Account of Flagship Conferences and Journals

Recent developments in AI, Machine Learning and Robotics have raised concerns about the ethical consequences of both academic and industrial AI research. Leading academics, businessmen and politicians have voiced an increasing number of questions about the consequences of AI not only over people, but also on the large-scale consequences on the the future of work and employment, its social consequences and the sustainability of the planet. In this work, we analyse the use and the occurrence of ethics-related research in leading AI, machine learning and robotics venues. In order to do so we perform long term, historical corpus-based analyses on a large number of flagship conferences and journals. Our experiments identify the prominence of ethics-related terms in published papers and presents several statistics on related topics. Finally, this research provides quantitative evidence on the pressing ethical concerns of the AI community.

==> tables/ranking-conferences.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|}
\hline
Ranking & Keyword & Count \\ \hline
\#1 & robot & 6794 \\ \hline
\#2 & learning & 6684 \\ \hline
\#3 & control & 6330 \\ \hline
\#4 & based & 4017 \\ \hline
\#5 & system & 3658 \\ \hline
\#6 & planning & 3245 \\ \hline
\#7 & robots & 3228 \\ \hline
\#8 & mobile & 2713 \\ \hline
\#9 & motion & 2530 \\ \hline
\#10 & model & 2418 \\ \hline
\#11 & approach & 2370 \\ \hline
\#12 & analysis & 2234 \\ \hline
\#13 & robotic & 2195 \\ \hline
\#14 & systems & 2187 \\ \hline
\#15 & design & 2106 \\ \hline
\#16 & dynamic & 2025 \\ \hline
\#17 & data & 1876 \\ \hline
\#18 & networks & 1829 \\ \hline
\#19 & models & 1798 \\ \hline
\#20 & visual & 1649 \\ \hline
\end{tabular}
\caption{Ranking of the 20 most popular keywords on paper titles of main AI and robotics conferences.}
\label{tab:ranking_keywords_conf}
\end{table}

==> tables/ranking-journals.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|}
\hline
Ranking & Keyword & Count \\ \hline
\#1 & systems & 19576 \\ \hline
\#2 & networks & 14938 \\ \hline
\#3 & analysis & 14070 \\ \hline
\#4 & control & 13578 \\ \hline
\#5 & design & 10112 \\ \hline
\#6 & system & 9711 \\ \hline
\#7 & based & 9364 \\ \hline
\#8 & data & 9302 \\ \hline
\#9 & algorithm & 9091 \\ \hline
\#10 & estimation & 8479 \\ \hline
\#11 & approach & 8197 \\ \hline
\#12 & model & 7609 \\ \hline
\#13 & detection & 7523 \\ \hline
\#14 & adaptive & 7213 \\ \hline
\#15 & performance & 7187 \\ \hline
\#16 & wireless & 6182 \\ \hline
\#17 & power & 6174 \\ \hline
\#18 & image & 6128 \\ \hline
\#19 & network & 5669 \\ \hline
\#20 & method & 5408 \\ \hline
\end{tabular}
\caption{Ranking of the 20 most popular keywords on paper titles of main AI and robotics journals.}
\label{tab:ranking_keywords_journal}
\end{table}

==> tables/results-conferences.tex <==
\begin{table}[h]
\label{tableresults_conferences_stats}
\scriptsize
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Year & AAAI & IJCAI & NIPS & ICML & ICRA & IROS \\ \hline
%81 & - 				& $0 / 0$			& - 			& - 			& - 			& - \\ \hline
%82 & $0 / 0$ 		& - 				& - 			& - 			& - 			& - \\ \hline
83 & $0 / 0$ 		& $.004 / 1$ 		& - 			& - 			& - 			& - \\ \hline
%84 & $0 / 0$ 		& - 				& - 			& - 			& $0 / 0$		& - \\ \hline
85 & - 				& $.008 / 2$ 		& - 			& - 			& $0 / 0$		& - \\ \hline
%86 & $0 / 0$ 		& - 				& - 			& - 			& $0 / 0$		& - \\ \hline
87 & $0 / 0$ 		& $0 / 0$			& $0 / 0$ 		& - 			& $.003/ 1$		& - \\ \hline
88 & $.007 / 1$ 	& - 				& $0 / 0$ 		& - 			& $.003/ 1$		& - \\ \hline
89 & - 				& $0 / 0$			& $0 / 0$ 		& - 			& $.004/ 1$		& $.011 / 1$ \\ \hline
%90 & $0 / 0$ 		& - 				& $0 / 0$ 		& - 			& - 			& $0 / 0$ \\ \hline
%91 & $0 / 0$ 		& $0 / 0$ 			& $0 / 0$ 		& - 			& - 			& $0 / 0$ \\ \hline
92 & $.007 / 1$ 	& - 				& $0 / 0$ 		& - 			& $.007/ 3$ 	& $.004 / 1$ \\ \hline
%93 & $0  / 0$ 		& $0 / 0$ 			& $0 / 0$ 		& $0/ 0$		& - 			& $0 / 0$ \\ \hline
94 & $.003 / 1$ 	& - 				& $0 / 0$ 		& $.023/ 1$		& $0 / 0$		& $0 / 0$ \\ \hline
95 & - 				& $0 / 0$ 			& $0 / 0$ 		& $0 / 0$		& $.004 / 2$	& - \\ \hline
%96 & - 				& - 				& $0 / 0$ 		& $0 / 0$		& $0 / 0$		& $0 / 0$ \\ \hline
97 & - 				& $.011 / 1$ 		& $0 / 0$ 		& $0 / 0$		& $0 / 0$		& $0 / 0$ \\ \hline
98 & - 				& - 				& $0 / 0$ 		& $0 / 0$		& $.002 / 1$	& $0 / 0$ \\ \hline
99 & - 				& $0 / 0$ 			& $.007 / 1$	& $0 / 0$		& $0 / 0$		& $0 / 0$ \\ \hline
00 & $0 / 0$		& - 				& $0 / 0$		& $.007/ 1$		& $.002 / 1$	& $0 / 0$ \\ \hline
01 & - 				& $0 / 0$ 			& $0 / 0$		& $0 / 0$		& $.003 / 2$	& $0 / 0$ \\ \hline
02 & - 				& - 				& $.005 / 1$ 	& $0 / 0$		& $.001 / 1$	& $0 / 0$ \\ \hline
03 & - 				& $.003 / 1$ 		& $.005 / 1$ 	& $0 / 0$		& $.006 / 4$	& $.003 / 2$ \\ \hline
04 & $1 / 2$ 		& - 				& $0 / 0$		& $0 / 0$		& $.002 / 2$	& $.002 / 1$ \\ \hline
05 & $0 / 0$ 		& $.011 / 4$		& $0 / 0$		& $0 / 0$		& $0 / 0$		& $.005 / 3$ \\ \hline
06 & $0.005 / 2$ 	& - 				& $.005 / 1$ 	& $0 / 0$		& $.004 / 3$	& $.003 / 3$ \\ \hline
07 & $0 / 0$ 		& $.004 / 2$		& $0 / 0$		& $0 / 0$		& $0 / 0$		& $.004 / 3$ \\ \hline
08 & $.017 / 6$ 	& - 				& $0 / 0$		& $0 / 0$		& $.003 / 2$	& $.003 / 2$ \\ \hline
09 & - 				& $0 / 0$ 			& $0 / 0$		& $0 / 0$		& $.003 / 2$	& $0 / 0$ \\ \hline
10 & $.006 / 2$ 	& - 				& $.003 / 1$ 	& $0 / 0$		& $.001 / 1$	& $.002 / 2$ \\ \hline
11 & $.019 / 6$ 	& $.01 / 5$ 		& $0 / 0$		& $0 / 0$		& $.002 / 2$	& $0 / 0$ \\ \hline
12 & $.011 / 4$ 	& - 				& $.003 / 1$ 	& $0 / 0$		& $0 / 0$		& $.001 / 1$ \\ \hline
13 & $.008 / 2$ 	& $.01 / 5$ 		& $.003 / 1$ 	& -				& $0 / 0$		& $0 / 0$ \\ \hline
14 & $.010 / 5$ 	& - 				& $.005 / 2$ 	& $0 / 0$		& $0 / 0$		& $0 / 0$ \\ \hline
15 & $.004 / 3$ 	& $.01 / 7$ 		& $.002 / 1$ 	& $.007/ 2$		& $0 / 0$		& $0 / 0$ \\ \hline
16 & $.017 / 12$ 	& $.004 / 3$		& $.005 / 3$ 	& $0 / 0$		& $.001 / 1$	& $.001 / 1$ \\ \hline
17 & $0.01 / 8$ 	& $.011 / 9$		& - 			& $.007/ 3$		& $.001 / 1$	& - \\ \hline
\end{tabular}
\caption{Average and total number of matches of the selected ethics-related keywords per year in paper titles for five leading AI (AAAI, IJCAI, NIPS, ICML) and Robotics (ICRA, IROS) conferences from $1981$ to $2017$. Omitted years had no occurrence of the keywords}
\end{table}

==> tables/results-journals.tex <==
\begin{table}[h]
\scriptsize
\centering
\begin{tabular}{|c|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|}
\hline
Year & ACM Trans. & Comm. ACM & IEEE Computer & JAIR & IEEE Trans. AI & Artif. Intell. \\ \hline
81 & $.00/ 0$	& $.00/ 0$	& $.00/ 0$	& -				& -				& $.00/ 0$ \\ \hline
82 & $.00/ 0$	& $.00/ 0$	& $.02/ 2$	& -				& -				& $.00/ 0$ \\ \hline
83 & $.00/ 0$	& $.00/ 0$	& $.00/ 0$	& -				& -				& $.03/ 1$ \\ \hline
84 & $.00/ 0$	& $.00/ 0$	& $.02/ 2$	& -				& -				& $.00/ 0$ \\ \hline
85 & $.00/ 0$	& $.00/ 0$	& $.00/ 0$	& -				& -				& $.00/ 0$ \\ \hline
86 & $.00/ 0$	& $.01/ 1$	& $.00/ 0$	& -				& -				& $.00/ 0$ \\ \hline
87 & $.01/ 1$	& $.00/ 0$	& $.01/ 1$	& -				& -				& $.00/ 0$ \\ \hline
88 & $.01/ 1$	& $.00/ 0$	& $.13/ 8$	& -				& -				& $.00/ 0$ \\ \hline
89 & $.00/ 0$	& $.00/ 0$	& $.08/ 8$	& -				& -				& $.02/ 1$ \\ \hline
90 & $.00/ 0$	& $.00/ 0$	& $.00/ 0$	& -				& .$26/ 9$ 		& $.03/ 2$ \\ \hline
91 & $.00/ 0$	& $.01/ 1$	& $.04/ 4$	& -				& $.30/ 22$ 	& $.00/ 0$ \\ \hline
92 & $.00/ 0$	& $.00/ 0$	& $.02/ 2$	& -				& $.32/ 33$ 	& $.01/ 1$ \\ \hline
93 & $.00/ 0$	& $.00/ 0$	& $.00/ 0$	& $.00/ 0$		& $.20/ 26$ 	& $.04/ 5$ \\ \hline
94 & $.00/ 1$	& $.03/ 4$	& $.00/ 0$	& $.00/ 0$		& $.17/ 22$ 	& $.02/ 2$ \\ \hline
95 & $.00/ 0$	& $.01/ 1$	& $.00/ 0$	& $.00/ 0$		& $.14/ 30$ 	& $.01/ 1$ \\ \hline
96 & $.00/ 0$	& $.00/ 0$	& $.06/ 8$	& $.00/ 0$		& $.20/ 41$ 	& $.00/ 0$ \\ \hline
97 & $.00/ 0$	& $.00/ 1$	& $.01/ 2$	& $.05/ 1$		& $.23/ 48$ 	& $.03/ 3$ \\ \hline
98 & $.01/ 3$	& $.00/ 0$	& $.00/ 0$	& $.00/ 0$		& $.23/ 47$ 	& $.04/ 4$ \\ \hline
99 & $.01/ 3$	& $.01/ 3$	& $.02/ 3$	& $.00/ 0$		& $.17/ 40$ 	& $.01/ 1$ \\ \hline
00 & $.01/ 2$	& $.00/ 0$	& $.01/ 2$	& $.00/ 0$		& $.12/ 28$ 	& $.01/ 1$ \\ \hline
01 & $.01/ 3$	& $.00/ 1$	& $.00/ 0$	& $.04/ 1$		& $.15/ 38$ 	& $.02/ 2$ \\ \hline
02 & $.02/ 6$	& $.00/ 1$	& $.00/ 1$	& $.00/ 0$		& $.15/ 39$ 	& $.03/ 2$ \\ \hline
03 & $.00/ 1$	& $.01/ 2$	& $.00/ 1$	& $.00/ 0$		& $.12/ 29$ 	& $.00/ 0$ \\ \hline
04 & $.00/ 1$	& $.00/ 1$	& $.01/ 2$	& $.00/ 0$		& $.13/ 32$ 	& $.02/ 1$ \\ \hline
05 & $.02/ 10$	& $.00/ 0$	& $.01/ 2$	& $.00/ 0$		& $.11/ 29$ 	& $.03/ 2$ \\ \hline
06 & $.01/ 5$	& $.00/ 0$	& $.02/ 6$	& $.00/ 0$		& $.10/ 47$ 	& $.00/ 0$ \\ \hline
07 & $.01/ 9$	& $.01/ 3$	& $.01/ 2$	& $.02/ 1$		& $.14/ 76$ 	& $.00/ 0$ \\ \hline
08 & $.01/ 6$	& $.00/ 0$	& $.00/ 0$	& $.03/ 2$		& $.15/ 78$ 	& $.00/ 0$ \\ \hline
09 & $.01/ 5$	& $.00/ 1$	& $.00/ 0$	& $.02/ 1$		& $.17/ 88$ 	& $.02/ 1$ \\ \hline
10 & $.00/ 2$	& $.01/ 2$	& $.00/ 0$	& $.00/ 0$		& $.05/ 32$ 	& $.00/ 0$ \\ \hline
11 & $.00/ 1$	& $.00/ 1$	& $.01/ 1$	& $.00/ 0$ 		& $.12/ 79$ 	& $.01/ 1$ \\ \hline
12 & $.01/ 9$	& $.00/ 1$	& $.00/ 0$	& $.02/ 1$ 		& $.10/ 74$ 	& $.00/ 0$ \\ \hline
13 & $.01/ 9$	& $.01/ 4$	& $.00/ 0$	& $.00/ 0$ 		& $.08/ 61$ 	& $.00/ 0$ \\ \hline
14 & $.01/ 16$	& $.00/ 0$	& $.01/ 2$	& $.00/ 0$ 		& $.12/ 77$ 	& $.02/ 1$ \\ \hline
15 & $.03/ 34$	& $.01/ 3$	& $.01/ 1$	& $.00/ 0$ 		& $.13/ 107$	& $.03/ 2$ \\ \hline
16 & $.03/ 43$	& $.02/ 5$	& $.01/ 2$	& $.02/ 1$ 		& $.10/ 78$ 	& $.01/ 1$ \\ \hline
17 & $.02/ 29$	& $.02/ 4$	& $.03/ 5$	& $.02/ 1$ 		& $.14/ 94$ 	& $.02/ 2$ \\ \hline
\end{tabular}
\label{tab:results_journals_stats}
\caption{Average and total number of matches of the selected ethics-related keywords per year in paper titles for six groups of the leading computing journals from $1981$ to $2017$. IEEE journals in AI are grouped into IEEE Trans. AI.}
\end{table}
